Test Suites as a Source of Training Data for Static Analysis Alert Classifiers

Flaw-finding static analysis tools typically generate large volumes of code flaw alerts including many false positives. To save on human effort to triage these alerts, a significant body of work attempts to use machine learning to classify and prioritize alerts. Identifying a useful set of training data, however, remains a fundamental challenge in developing such classifiers in many contexts. We propose using static analysis test suites (i.e., repositories of "benchmark" programs that are purpose-built to test coverage and precision of static analysis tools) as a novel source of training data. In a case study, we generated a large quantity of alerts by executing various static analyzers on the Juliet C/C++ test suite, and we automatically derived ground truth labels for these alerts by referencing the Juliet test suite metadata. Finally, we used this data to train classifiers to predict whether an alert is a false positive. Our classifiers obtained high precision (90.2%) and recall (88.2%) for a large number of code flaw types on a hold-out test set. This preliminary result suggests that pre-training classifiers on test suite data could help to jumpstart static analysis alert classification in data-limited contexts.

==> Makefile <==
#
# Makefile for paper
#

PACKAGE=IEEEtran

PAPER = rapidclass.tex 

PDF = ${PAPER:%.tex=%.pdf} rapidclass.pdf

all:  ${PDF}

%.pdf:  %.tex   $(PACKAGE).cls IEEEtran.bst *.tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx
	pdflatex $<


rapidclass.pdf: rapidclass-body-conf.tex sections/classifiers_build_and_test.tex tables/* figs/*

.PRECIOUS:  $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) 



==> mathmode-spacing.tex <==
% Source: http://tex.stackexchange.com/a/129454
% Adjusts spacing between letters in math mode for multiple-letter identifiers.

\usepackage{etexcmds}

\makeatletter
\newtoks\m@toks@math
\newtoks\m@toks@text

\edef\m@tmp@restore{%
  \lccode\number`\X=\the\lccode`\X\relax
  \lccode\number`\~=\the\lccode`\~\relax
}

\newcommand*{\m@activate}{}
\newcommand*{\m@check@letter}{}
\newcommand*{\m@check@fi}{}

\newif\ifm@single

\let\m@start\relax
\def\m@loop{%
  \lccode`\X=\count@
  \lccode`\~=\count@
  \lowercase{%
    \expandafter\mathchardef\csname m@code@X\endcsname=\mathcode\count@
    \edef\m@activate{%
      \etex@unexpanded\expandafter{\m@activate}%
      \mathcode\the\count@="8000\relax
      \def\noexpand~{\m@start\csname m@code@X\endcsname X}%
    }%
    \g@addto@macro\m@check@letter{%
      \ifx\@let@token X\else
    }%
  }%
  \g@addto@macro\m@check@fi{\fi}%
  \advance\count@\@ne
}
% A-Z
\count@=`\A\relax
\@whilenum\count@<\numexpr`\Z+1\relax\do{\m@loop}
% a-z
\count@=`\a\relax
\@whilenum\count@<\numexpr`\z+1\relax\do{\m@loop}

\newcommand*{\m@start}[2]{%
  \bgroup
  \m@toks@math{#1}%
  \m@toks@text{#2}%
  \m@singletrue
  \futurelet\@let@token\m@check
}
\edef\m@check{%
  \etex@unexpanded{%
    \let\m@next\m@add
    \ifx\@let@token\space
      \let\m@next\m@finish
    \else
      \ifx\@let@token\egroup
        \let\m@next\m@finish
      \else
  }%
  \etex@unexpanded\expandafter{%
        \m@check@letter
  }%
  \etex@unexpanded{%
          \let\m@next\m@finish
  }%
  \etex@unexpanded\expandafter{%
        \m@check@fi
  }%
  \etex@unexpanded{%
      \fi
    \fi
    \m@next
  }%
}

\newcommand*{\m@add}[1]{%
  \m@singlefalse
  \m@toks@math\expandafter{%
    \the\expandafter\m@toks@math
    \csname m@code@#1\endcsname
  }%
  \m@toks@text\expandafter{%
    \the\m@toks@text
    #1%
  }%
  \futurelet\@let@token\m@check
}

\newcommand*{\m@finish}{%
  \ifm@single
    \expandafter\mprintsingle\expandafter{%
      \the\expandafter\m@toks@math\expandafter
    }\expandafter{%
      \the\expandafter\m@toks@text\expandafter
    }%
  \else
    \expandafter\mprintmulti\expandafter{%
      \the\expandafter\m@toks@math\expandafter
    }\expandafter{%
      \the\expandafter\m@toks@text\expandafter
    }%
  \fi
  \egroup
}
\let\mprintsingle\@firstoftwo
\let\mprintmulti\@firstoftwo

\everymath{\m@activate}
\everydisplay{\m@activate}

\m@tmp@restore
\makeatother

\renewcommand*{\mprintsingle}[2]{{#1}}%
\renewcommand*{\mprintmulti}[2]{\mathit{#1}}%


==> snippets/n_CWE_in_test_set.tex <==
%DO NOT EDIT DIRECTLY! Autoproduced in /zkurtz/classify/ophelia/publish/compile_results_for_icse2019.R
79

==> snippets/training_counts_statement.tex <==
%DO NOT EDIT DIRECTLY! Autoproduced in /zkurtz/classify/ophelia/publish/compile_results_for_icse2019.R
36,968 TP meta alerts and 84,269 FP meta alerts.

==> tables/feature_importance_raw.tex <==
% latex table generated in R 3.4.3 by xtable 1.8-2 package
% Fri Mar  9 13:23:48 2018
\begin{table}[ht]
\centering
\begin{tabular}{rlr}
  \hline
Rank & Feature & Gain \\ 
  \hline
  1 & function\_ccsm\_FUNC\_CALLED\_BY\_LOCAL & 0.42 \\ 
    2 & checker\_id & 0.28 \\ 
    3 & file\_und\_CountLineInactive & 0.04 \\ 
    4 & file\_ccsm\_KW\_CUM\_STATIC\_CNT & 0.04 \\ 
    5 & function\_und\_CountInput & 0.03 \\ 
    6 & cwe & 0.02 \\ 
    7 & function\_lizard\_params & 0.01 \\ 
    8 & function\_und\_CountPath & 0.01 \\ 
    9 & function\_und\_Knots & 0.01 \\ 
   10 & function\_und\_CountLine & 0.01 \\ 
   \hline
\end{tabular}
\caption{Top 10 features based on total information gain in LightGBM} 
\label{table:feature_importance}
\end{table}


==> tables/speculative_100.tex <==
%\begin{table}[ht]
\begin{table}[htbp]
\centering
\begin{tabular}{lrrrr}
  \hline
Model & Accuracy & Precision & Recall & AUROC \\ 
  \hline
  LightGBM & 0.93928 & 0.92944 & 0.92982 & 0.99247 \\
  xgboost  & 0.92538 & 0.89949 & 0.90291 & 0.98773 \\
  random forest & 0.91271 & 0.91715 & 0.9055 & 0.96906 \\
  lasso & 0.89887 & 0.86894 & 0.87278 & 0.97577 \\
   \hline
\end{tabular}
\caption{Performance summary with speculatively mapped alerts, $100\%$ threshold.} 
\label{table:speculative_100}
\end{table}


==> tables/speculative_50.tex <==
%\begin{table}[ht]
\begin{table}[htbp]
\centering
\begin{tabular}{lrrrr}
  \hline
Model & Accuracy & Precision & Recall & AUROC \\ 
  \hline
  LightGBM & 0.9416 & 0.92885 & 0.93089 & 0.99302 \\
  xgboost & 0.93028 & 0.9003 & 0.90081 & 0.98899 \\
  random forest & 0.91833 &  0.91073 & 0.91007 & 0.97064 \\
  lasso & 0.90309 & 0.87417 & 0.87816 & 0.9786 \\ 
   \hline
\end{tabular}
\caption{Performance summary with speculatively mapped alerts, $50\%$ threshold.} 
\label{table:speculative_50}
\end{table}


==> tables/speculative_75.tex <==
%\begin{table}[ht]
\begin{table}[htbp]
\centering
\begin{tabular}{lrrrr}
  \hline
Model & Accuracy & Precision & Recall & AUROC \\ 
  \hline
  LightGBM & 0.93779 & 0.92809 & 0.92711 & 0.99223 \\
  xgboost  & 0.92224 & 0.89907 & 0.89912 & 0.98669 \\
  random forest & 0.91563 & 0.91763 & 0.91078 & 0.96915 \\
  lasso & 0.89695 & 0.87309 & 0.87415 & 0.97529 \\ 
   \hline
\end{tabular}
\caption{Performance summary with speculatively mapped alerts, $75\%$ threshold.} 
\label{table:speculative_75}
\end{table}

